Multiple Models for Recommending Temporal Aspects of Entities

Entity aspect recommendation is an emerging task in semantic search that helps users discover serendipitous and prominent information with respect to an entity, of which salience (e.g., popularity) is the most important factor in previous work. However, entity aspects are temporally dynamic and often driven by events happening over time. For such cases, aspect suggestion based solely on salience features can give unsatisfactory results, for two reasons. First, salience is often accumulated over a long time period and does not account for recency. Second, many aspects related to an event entity are strongly time-dependent. In this paper, we study the task of temporal aspect recommendation for a given entity, which aims at recommending the most relevant aspects and takes into account time in order to improve search experience. We propose a novel event-centric ensemble ranking method that learns from multiple time and type-dependent models and dynamically trades off salience and recency characteristics. Through extensive experiments on real-world query logs, we demonstrate that our method is robust and achieves better effectiveness than competitive baselines.

==> queryset.tex <==
\section{Data Set}
\label{sec:queryset}
\subsection{Query logs}
We used two query log datasets in this study. The first dataset is the AOL query logs, 
which consists of more than 30 million queries covering the period from 1 March to 31 May 2006.
The second dataset we used is the MSN query logs\footnote{{\scriptsize \url{http://research.microsoft.com/~nickcr/wscd09/}}} 
composed of about 15 million queries sampled from May 2006. User information is anonymized and adult search queries are ignored from the study.
We followed data filtering steps suggested in~\cite{Zhu:2011:UFR:1963405.1963415} as follows: 1)~remove all non-English queries, 
2)~convert queries into lower case, 3)~ignore queries with frequency less than 5 (for filtering noisy data), 
4)~ignore those with frequency more than 15,000 (i.e., navigational queries, which are not useful for our study), 
and 5)~remove click-through data with frequency less than 3.
%The statistics for both datasets under non- and filtering conditions are shown in Table~\ref{tab:datasets}.

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[tbp]
  \label{tab:datasets}%
  \centering
  {\scriptsize
  \caption{Statistics of two query log datasets.}
    \begin{tabular}{lrrrr}
		\toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{2}{c}{AOL} & \multicolumn{2}{c}{MSN} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Raw} & \multicolumn{1}{c}{Filtered} & \multicolumn{1}{c}{Raw} & \multicolumn{1}{c}{Filtered} \\\midrule
    \#queries & 33,944,630 & 18,614,850 & 14,844,988 & 6,015,318 \\
    \#unique queries & 9,536,327 & 1,087,259 & 6,344,840 & 268,271 \\
    \#unique URLs & 1,572,102 & 545,223 & 4,973,603 & 788,441 \\
    \#clicks & 18,198,017 & 1,689,712 & 13,987,165 & 4,894,418 \\
    \bottomrule
    \end{tabular}%
  }
\end{table}%
 
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table}[htbp]
%  \centering
%  {\scriptsize
%  \caption{Statistics of temporal queries identified as \textit{explicit} and \textit{implicit}.%, and \textit{event-related} queries chosen for evaluating query recommendation.
%  }
%    \begin{tabular}{crrr}
%    \toprule
%    \multicolumn{2}{c}{Query Type} & \multicolumn{1}{c}{AOL} & \multicolumn{1}{c}{MSN} \\
%    \midrule
%    \multirow{3}[0]{*}{Explicit} & \multicolumn{1}{l}{\#queries} & 19531 & 2728 \\
%          & \multicolumn{1}{l}{\#labeled} & 4994  & 2728 \\
%          & \multicolumn{1}{l}{\#events} & 256   & 159 \\ \midrule
%    \multirow{3}[0]{*}{Implicit} & \multicolumn{1}{l}{\#clusters} & 121176 & 17009 \\
%          & \multicolumn{1}{l}{\#labeled} & 710   & 318 \\
%          & \multicolumn{1}{l}{\#events} & 305   & 159 \\ %\midrule
%    %\multirow{2}[0]{*}{Recommendation} & \multicolumn{1}{l}{\#queries} & 65    & 23 \\
%    %      & \multicolumn{1}{l}{\#labeled} & 65    & 23 \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{tab:labelstats}%
%\end{table}%

\subsection{Event-related queries}

There is no standard dataset available for event-related queries that can be used in our study. 
%We employed the proposed method in Section~\ref{sec:eventextraction} to 
In the following, we explain our method for identifying event-related queries from the query logs of AOL and MSN. 
%\section{Event-related Query Identification}
%\label{sec:eventextraction}
%In this section, we propose approaches to identifying 
First, we determine two types of event-related queries, namely, \textit{explicit} and \textit{implicit} queries.

\textbf{Explicit Query}
Explicit event-related queries will be determined by temporal expressions mentioned in queries, which can be automatically 
extracted using a time and event recognition algorithm. The algorithm extracts temporal expressions mentioned in a document and normalizes them to dates so
they can be anchored on a timeline. A temporal expression can be either explicit (e.g., 2006 in \textsf{World Cup 2006} or implicit (e.g., \textsf{Independent Day}). 
%As explained in~\cite{DBLP:conf/cikm/AlonsoGB09}, temporal expressions can be explicit, implicit or relative. Examples of explicit temporal expressions are \textsf{May 25, 2012} or \textsf{June 17, 2011} that can be mapped directly to dates months, or years on the Gregorian calendar.  An implicit temporal expression is an imprecise time point or interval, e.g.,  \textsf{Independence Day 2011} that can be mapped to \textsf{July 04, 2011}. Examples of relative temporal expressions are \textsf{yesterday}, \textsf{last week} or \textsf{one month ago}. 
Recent work~\cite{Campos:2012:GDS:2396761.2398567,KanhabuaRS12} has shown that temporal expressions %,StrotgenAG12
identified might be \textit{not equally relevant} or \textit{irrelevant} to a given event. We hence choose them as the candidates for studying.

%Thus, the identified explicit queries will be classified further as event-related or not. The proposed features for query classification will be presented in Section~\ref{subsec:classification}.

\textbf{Implicit Query}
%{\color{red} this clustering technique is questioned about the feasibility for real-time application, we should change to clearly address that this is the pre-processing step for detecting event-related queries. We can say that this can be used as training data as for later event-related queries classification, but for simplicity of the work, we omit this in this paper.}
A large amount of event-related queries has no explicit temporal expressions. Such implicit queries can be detected using a time series analysis, 
in which the time series data of a query, i.e., query volume over time, will be created for conducting a time series analysis.
However, aggregating the frequency over time for each individual query is limited due to data sparsity. Thus, we tackle this problem by means of finding clusters of related queries.
More precisely, we employ a cluster technique to group queries related to the same event, and use the volume aggregated from query members in the cluster for the time series analysis. Note that, this clustering step is only a quality enhancement phase in the preprocessing step. We can of course study on the individual query, however, to detect highly accurate implicit queries for our study, we chose to conduct the technique.
%As described in~\cite{2002:QCU:503104.503108}, existing query clustering methods are based on two ways: using query keywords, or query-URL bipartite graphs. 
%In this work, we use only query keywords, and clustering millions of queries can be infeasible in term of time computation. 
We  perform a \textit{keyword}-based query clustering in two main steps as follows.

\textbf{Step 1:} We extract all distinct queries in the dataset. Clustering queries in the whole dataset can result in grouping query keywords unrelated to the same event. We account for noisy data by assuming that partition the dataset by time will increase the accuracy of finding related event queries. We believe the fact that queries of an event can significantly peak with regards to frequency only in a short period (days). 

\textbf{Step 2:} On the sets of queries grouped by time partitioning method, we lowercased all query terms and sort the queries alphabetically. We defined the pair of sorted queries that stand next to each other are \textit{adjacent} queries. Every \textit{adjacent} query pair was preprocessed (stop-word removed and Porter-stemmed)  and computed with Jaccard Similarity then putting in the same cluster if the similarity score is over a defined threshold. The cluster statistics are then exploited for choosing event-related query candidates.


In total, we identified 837 event-related queries, where a query is event-related if it refers to or related to a real-world event happening in the past, present or future. Following the taxonomy of event-related queries presented in~\cite{DBLP:conf/icwsm/KairamMTLD13}, we manually classified the identified queries into five distinct subtypes (i.e., \textsf{Breaking}, \textsf{Ongoing}, \textsf{Meme}, \textsf{Commemorative} and \textsf{Anticipated}), with respect to the time span of the query logs datasets. In our settings, \textsf{Breaking} points to unplanned events, \textsf{Ongoing} indicates happening events along the query log period while \textsf{Meme} implies a viral phenomenon and \textsf{Commemorative} refers to past events. We introduced a new subtype \textsf{Anticipated} for a specific subtype of our query logs, which indicates \textit{high impact, future} events, such as, sport competitions, holidays or festivals that people start searching for them sometimes before the event starts. We further labels the events into eight different topics (i.e., \textit{News}, \textit{Fact}, \textit{Entertainment}, \textit{Politics}, \textit{Celebrity}, \textit{Sports}, \textit{Holidays}, and \textit{Deaths}). The statistics of our event-related queries classified by subtypes and topics are shown in Figure~\ref{fig:ma}. 
%
%\begin{figure}[t]
%\centering
%		\includegraphics[width=0.45\textwidth]{images/queries_by_subtypes.eps}\vspace{-0.1cm}
%		\caption{Event-related queries classified by subtypes.}
%		\label{fig:querysubtypes}
%\end{figure}
%%\vspace{-0.1cm}
%
%\begin{figure}[t]
%\centering
%		\includegraphics[width=0.45\textwidth]{images/queries_by_topics.eps}\vspace{-0.1cm}
%		\caption{Event-related queries classified by topics.}
%		\label{fig:querytopics}
%\end{figure}
%%\vspace{-0.1cm}

% - Settings:
% 	- Time-aware Annotation: ``dynamic labels'', 1: fuzzy, -1: not judged; no queries labeled as -1 in the filtering case (only queries that are above threshold for JC and Edit dist are labelled / merge queries generated from knn and rwrw for labelling)
%		- Examples of query labels / Temporal distribution of queries in different bins of retrieval performance / Statistics for number of candidates per queries and number of improved candidates (see adaptive SIGIR'12 paper)
%		- Statistics about graph datasets
\subsection{Dynamic relevance assessment}

To study our query recommendation task, we manually selected trending events composed of queries from three subtypes: \textsf{Breaking}, \textsf{Ongoing}, and \textsf{Anticipated}. We performed \textit{time-aware assessment} in order to obtain relevance judgments for a list of query recommendations generated for each trending event. Time-aware assessment refers to the annotation process taking into account \textit{dynamic relevance}, i.e., the relevance label of a recommendation for a given event is varied; depending on when it was issued with respect to the event time. For instance, the suggestion \textsf{world cup tickets} is highly relevant \textbf{before} the happening of an event query \textbf{world cup 2006}, and it becomes less relevant  \textbf{after} the event, whereas \textsf{world cup results} or \textsf{world cup final} are more relevant in the \textbf{during} or \textbf{after} event periods.
Our time-aware annotation process was conducted as follows. In total, there were 65 trending events. For each trending event, we merged the top-ranked list of candidate suggestion queries generated by two state-of-the-art query recommendation methods (K-Nearest Neighbors and Random Walk on co-clicked query-URL graph). The list of candidates contained many near-duplicate or noisy data, hence we removed near-redundancy candidates based on text similarity metrics (i.e., Jaccard similarity and edit distance) using specific thresholds observed empirically. For a pair of event and a candidate suggestion was judged by at least two human assessors. The relevance labeling criteria is as follows. Human assessors were asked to evaluate event/suggestion pair (as relevant or non-relevant) with respect to \textit{three main periods}, namely, periods \textbf{before}, \textbf{during}, and \textbf{after} for a given event.
Particularly, an assessor gave a relevance score $Grade(q,s,t)$ where $(q,s,t)$ is a triple of a query $q$, a suggestion $s$, and an event period $t$.
We defined 4 levels of relevance: 3 for \textit{excellent} (very relevant suggestion), 2 for \textit{good} (relevant suggestion), 
1 for \textit{bad} (non-relevant suggestion), and 0 for \textit{don't know} (not sure about it). All labels with the score 0 were excluded from the evaluation.
Finally, assessors evaluated 1,084 event/suggestion pairs (approximately 3,252 of triples), where there were approximately 17 suggestions per trending event on average. Examples of trending events and suggestions with dynamic labels are shown in Table~\ref{tab:dynamiclabel}.
Note that, the evaluated queries were taken from AOL query logs only because of its longer time span and the trending events in MSN logs are very similar and almost identical with AOL queries. Our labeled dataset is publicly available for download at\footnote{{\scriptsize \url{http://--REMOVE-FOR-BLIND-REVIEW--}.}}.

% Table generated by Excel2LaTeX from sheet 'Example'
\begin{table}[htbp]
{\scriptsize
  \centering
  \caption{Examples of trending events and the time-aware assessment for query suggestions (+ indicates that each suggestion has its original query as a prefix).}
    \begin{tabular}{llccr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[0]{*}{Event}} & \multicolumn{1}{c}{\multirow{2}[0]{*}{Suggestion}} & \multicolumn{3}{c}{Dynamic Label} \\ 
          &       & Before & During & After \\    \midrule
    american idol & + auditions & VR & R & NR \\
    american idol & + live tickets & R & R & NR \\
    american idol & + vote results & NR & VR & R \\
    american idol & + finale & NR & R & VR \\
    american idol & + reviews & NR & R & R \\    \midrule
    cinco de mayo & + pictures & VR & R & R \\
    cinco de mayo & + recipes & VR & R & R \\
    cinco de mayo & + activities & VR & R & NR \\
    cinco de mayo & + celebration & VR & R & NR \\   \midrule
    kentucky derby & + odds & VR & VR & R \\
    kentucky derby & + contenders & VR & R & R \\
    kentucky derby &  + winner & NR & VR & VR \\
    kentucky derby & + results & NR & VR & VR \\   \midrule
    mother's day & + cards & VR & R & NR \\
    mother's day & + gifts & VR & R & NR \\
    mother's day & + pictures & VR & R & R \\
    mother's day & + history & R & R & R \\   \midrule
    ncaa tournament & + picks & VR & R & NR \\
    ncaa tournament & + brackets & R & R & R \\
    ncaa tournament & + scores & NR & VR & R \\
    ncaa tournament & + champions & NR & R & VR \\
    ncaa tournament & + final four & NR & R & R \\   \midrule
    world cup & + schedule & VR & VR & NR \\
    world cup & + tickets & VR & R & NR \\
    \bottomrule
    \end{tabular}%
  \label{tab:dynamiclabel}%
  }
\end{table}%

% 	- Parameters for preprocessing (JC, Edit dist, n-gram overlap), temporal feature parameters, and training data partition strategies (randomized, n-fold, models and metrics used) for L2R algorithms
% 	- Metrics: formulas and explanation for ERR and NDCG; final results are the combination of two folds(not an average)
% 	- Methods for comparison: different L2R models learned using the proposed features, where baselines are default ranking using only semantic relatedness scores
%		- Note about the assignment of QIDs for training L2R algorithms using two methods:
%			1) Use the identical ID for each event query: possible to compare the performance among different ``fix'' hitting time points only, where the traning models of different ranked lists with the same QID can be unpredictable for event-based hiting normalization
%			2) Use (event ID, hitting time) as QID: possible to compare across event-based hitting time (treat the same event issued at different time points as distinct queries in training) 


\begin{figure}
\makebox[\columnwidth][c]{
%\begin{subfigure}[b]{.5\columnwidth}
%\centering\includegraphics[width=.95\columnwidth]{images/queries_by_subtypes.eps}
%\end{subfigure}
\begin{subfigure}[b]{.9\columnwidth}
\centering\includegraphics[width=.95\columnwidth]{images/queries_by_topics.png}
\end{subfigure}
}
\caption{Statistics of trending events manually annotated.}
\label{fig:ma}
\end{figure}

\begin{figure*}[t]
\makebox[\textwidth][c]{%
\begin{subfigure}[b]{.3\textwidth}
\centering\includegraphics[width=.9\columnwidth]{images/QueryDist_all_fix_knn.eps}
\end{subfigure}
\begin{subfigure}[b]{.3\textwidth}
\centering\includegraphics[width=.9\columnwidth]{images/QueryDist_all_fix_rwrw.eps}
\end{subfigure}
\begin{subfigure}[b]{.3\textwidth}
\centering\includegraphics[width=.9\columnwidth]{images/QueryDist_all_event_knn.eps}
\end{subfigure}
}
\caption{The distribution of trending events over time.}
\label{fig:dist}
\end{figure*}

==> rwrw_all_fix.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{rrrrrrrrrr}
    \toprule
    rwrw\_all\_2006-03-07\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-03-07\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    \midrule
    rwrw  & 0.09  & 0.37  & 0.37  & 0.37  & rwrw  & 0.5   & 0.82  & 0.82  & 0.82 \\
    CA + countBurst & 0.56 (+500\%) & 0.6 (+64\%) & 0.6 (+64\%) & 0.6 (+64\%) & CA + countBurst & 1 (+100\%) & 1 (+23\%) & 1 (+23\%) & 1 (+23\%) \\
    CA + timeDist & 0.56 (+500\%) & 0.6 (+64\%) & 0.6 (+64\%) & 0.6 (+64\%) & CA + timeDist & 1 (+100\%) & 1 (+23\%) & 1 (+23\%) & 1 (+23\%) \\
    LR + ALL & 0.09 (0\%) & 0.37 (0\%) & 0.37 (0\%) & 0.37 (0\%) & LR + ALL & 0.5 (0\%) & 0.82 (0\%) & 0.82 (0\%) & 0.82 (0\%) \\
    rwrw\_all\_2006-03-14\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-03-14\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.14  & 0.27  & 0.3   & 0.3   & rwrw  & 0.64  & 0.76  & 0.83  & 0.86 \\
    AR + ALL & 0.13 (-7\%) & 0.3 (+10\%) & 0.31 (+3\%) & 0.31 (+2\%) & AR + ALL & 0.48 (-26\%) & 0.8 (+6\%) & 0.81 (-1\%) & 0.83 (-4\%) \\
    CA + countBurst & 0.26 (+80\%) & 0.38 (+39\%) & 0.39 (+31\%) & 0.39 (+29\%) & CA + accEDecayCE & 0.77 (+19\%) & 0.86 (+13\%) & 0.91 (+10\%) & 0.92 (+8\%) \\
    CA + ALL & 0.21 (+44\%) & 0.31 (+15\%) & 0.33 (+10\%) & 0.33 (+10\%) & CA + avgDecayCE & 0.77 (+19\%) & 0.86 (+13\%) & 0.91 (+10\%) & 0.92 (+8\%) \\
    LR + countBurst & 0.26 (+80\%) & 0.38 (+39\%) & 0.39 (+31\%) & 0.39 (+29\%) & CA + ALL & 0.58 (-10\%) & 0.76 (+0\%) & 0.81 (-2\%) & 0.85 (-0\%) \\
    LR + ALL & 0.35 (+145\%) & 0.42 (+55\%) & 0.43 (+45\%) & 0.44 (+44\%) & LR + ALL & 0.71 (+10\%) & 0.85 (+12\%) & 0.88 (+7\%) & 0.89 (+4\%) \\
    rwrw\_all\_2006-03-21\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-03-21\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.21  & 0.36  & 0.39  & 0.4   & rwrw  & 0.64  & 0.73  & 0.77  & 0.84 \\
    AR + ALL & 0.38 (+76\%) & 0.47 (+31\%) & 0.5 (+29\%) & 0.5 (+26\%) & AR + ALL & 0.64 (0\%) & 0.79 (+8\%) & 0.86 (+12\%) & 0.86 (+3\%) \\
    CA + avgDecayCE & 0.55 (+159\%)* & 0.59 (+63\%)** & 0.6 (+54\%)** & 0.6 (+51\%)** & CA + avgDecayCE & 1 (+56\%)* & 0.94 (+28\%)** & 0.95 (+24\%)** & 0.97 (+16\%)** \\
    CA + ALL & 0.35 (+65\%) & 0.48 (+32\%) & 0.49 (+27\%) & 0.5 (+24\%) & CA + ALL & 0.65 (+2\%) & 0.81 (+10\%) & 0.83 (+8\%) & 0.87 (+4\%) \\
    LR + avgDecayCE & 0.55 (+159\%)* & 0.59 (+63\%)** & 0.6 (+54\%)** & 0.6 (+51\%)** & LR + avgDecayCE & 1 (+56\%)* & 0.94 (+28\%)** & 0.95 (+24\%)** & 0.97 (+16\%)** \\
    LR + ALL & 0.35 (+65\%) & 0.48 (+32\%) & 0.49 (+27\%) & 0.5 (+24\%) & LR + ALL & 0.65 (+2\%) & 0.81 (+10\%) & 0.83 (+8\%) & 0.87 (+4\%) \\
    rwrw\_all\_2006-03-31\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-03-31\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.19  & 0.31  & 0.34  & 0.35  & rwrw  & 0.64  & 0.74  & 0.8   & 0.85 \\
    AR + timeDist & 0.36 (+91\%)* & 0.44 (+41\%) & 0.45 (+32\%) & 0.46 (+31\%) & AR + ALL & 0.57 (-11\%) & 0.67 (-9\%) & 0.76 (-5\%) & 0.81 (-5\%) \\
    AR + ALL & 0.25 (+32\%) & 0.33 (+7\%) & 0.37 (+8\%) & 0.38 (+8\%) & CA + ALL & 0.81 (+26\%) & 0.78 (+5\%) & 0.84 (+6\%) & 0.9 (+6\%) \\
    CA + ALL & 0.37 (+97\%)* & 0.44 (+44\%)* & 0.46 (+34\%)* & 0.47 (+34\%)* & LR + minDuration & 0.83 (+29\%)* & 0.84 (+14\%) & 0.87 (+9\%) & 0.92 (+8\%) \\
    LR + timeDist & 0.38 (+103\%) & 0.47 (+51\%)* & 0.48 (+39\%)* & 0.49 (+38\%)* & LR + ratio & 0.84 (+30\%) & 0.84 (+13\%)** & 0.89 (+12\%)** & 0.92 (+8\%)*** \\
    LR + ALL & 0.31 (+67\%) & 0.41 (+32\%) & 0.43 (+24\%) & 0.44 (+24\%) & LR + ALL & 0.71 (+10\%) & 0.77 (+4\%) & 0.82 (+3\%) & 0.88 (+3\%) \\
    rwrw\_all\_2006-04-07\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-04-07\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.27  & 0.37  & 0.39  & 0.39  & rwrw  & 0.66  & 0.77  & 0.8   & 0.82 \\
    AR + accHDecayFreq & 0.37 (+36\%)* & 0.41 (+13\%) & 0.44 (+14\%) & 0.44 (+14\%) & AR + ALL & 0.7 (+6\%) & 0.69 (-10\%) & 0.8 (-1\%) & 0.83 (+1\%) \\
    AR + ALL & 0.35 (+29\%) & 0.4 (+8\%) & 0.42 (+10\%) & 0.43 (+10\%) & CA + accHDecayFreq & 0.79 (+20\%) & 0.76 (-1\%) & 0.85 (+6\%) & 0.87 (+6\%) \\
    CA + accHDecayFreq & 0.37 (+36\%)* & 0.41 (+13\%) & 0.44 (+14\%) & 0.44 (+14\%) & CA + ALL & 0.73 (+11\%) & 0.76 (-1\%) & 0.81 (+2\%) & 0.86 (+4\%) \\
    CA + ALL & 0.32 (+18\%) & 0.4 (+9\%) & 0.41 (+7\%) & 0.42 (+8\%) & LR + minDuration & 0.76 (+16\%) & 0.83 (+9\%) & 0.86 (+8\%) & 0.88 (+7\%) \\
    LR + ALL & 0.18 (-34\%) & 0.31 (-17\%) & 0.32 (-16\%) & 0.33 (-15\%) & LR + ALL & 0.58 (-12\%) & 0.72 (-6\%) & 0.79 (-2\%) & 0.81 (-2\%) \\
    rwrw\_all\_2006-04-14\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-04-14\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.26  & 0.36  & 0.38  & 0.39  & rwrw  & 0.57  & 0.71  & 0.76  & 0.78 \\
    AR + ALL & 0.19 (-24\%) & 0.29 (-18\%) & 0.33 (-13\%) & 0.34 (-13\%) & AR + ALL & 0.47 (-17\%) & 0.61 (-14\%) & 0.7 (-7\%) & 0.73 (-7\%) \\
    CA + maxDuration & 0.32 (+23\%) & 0.38 (+7\%) & 0.42 (+9\%) & 0.42 (+9\%) & CA + timeDist & 0.64 (+13\%) & 0.76 (+7\%) & 0.79 (+5\%) & 0.82 (+6\%) \\
    CA + ALL & 0.15 (-40\%) & 0.29 (-20\%) & 0.31 (-19\%) & 0.32 (-18\%) & CA + ALL & 0.52 (-8\%) & 0.63 (-12\%) & 0.71 (-6\%) & 0.76 (-3\%) \\
    LR + maxDuration & 0.32 (+23\%) & 0.38 (+7\%) & 0.42 (+9\%) & 0.42 (+9\%) & LR + maxDuration & 0.61 (+8\%) & 0.69 (-3\%) & 0.78 (+3\%) & 0.8 (+2\%) \\
    LR + ALL & 0.2 (-21\%) & 0.3 (-17\%) & 0.34 (-12\%) & 0.34 (-12\%) & LR + ALL & 0.51 (-11\%) & 0.64 (-11\%) & 0.74 (-3\%) & 0.76 (-3\%) \\
    rwrw\_all\_2006-04-21\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-04-21\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.24  & 0.36  & 0.38  & 0.39  & rwrw  & 0.67  & 0.75  & 0.79  & 0.8 \\
    AR + ALL & 0.22 (-9\%) & 0.31 (-14\%) & 0.33 (-14\%) & 0.34 (-11\%) & AR + ALL & 0.52 (-23\%) & 0.63 (-16\%)* & 0.69 (-12\%)* & 0.73 (-9\%)* \\
    CA + maxDuration & 0.34 (+40\%) & 0.4 (+12\%) & 0.43 (+12\%) & 0.44 (+13\%) & CA + maxDuration & 0.7 (+4\%) & 0.73 (-3\%) & 0.8 (+2\%) & 0.83 (+3\%) \\
    CA + ALL & 0.19 (-22\%) & 0.32 (-10\%) & 0.34 (-12\%) & 0.35 (-10\%) & CA + ALL & 0.49 (-26\%)* & 0.68 (-9\%) & 0.72 (-8\%) & 0.74 (-8\%) \\
    LR + maxDuration & 0.34 (+40\%) & 0.4 (+12\%) & 0.43 (+12\%) & 0.44 (+13\%) & LR + maxDuration & 0.7 (+4\%) & 0.73 (-3\%) & 0.8 (+2\%) & 0.83 (+3\%) \\
    LR + ALL & 0.22 (-11\%) & 0.32 (-11\%) & 0.35 (-9\%) & 0.35 (-9\%) & LR + ALL & 0.5 (-26\%) & 0.66 (-12\%) & 0.73 (-8\%) & 0.74 (-7\%) \\
    rwrw\_all\_2006-04-30\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-04-30\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.21  & 0.32  & 0.34  & 0.34  & rwrw  & 0.5   & 0.65  & 0.72  & 0.75 \\
    AR + ALL & 0.25 (+17\%) & 0.35 (+8\%) & 0.37 (+8\%) & 0.37 (+8\%) & AR + ALL & 0.59 (+18\%) & 0.7 (+8\%) & 0.76 (+5\%) & 0.78 (+5\%) \\
    CA + ALL & 0.24 (+16\%) & 0.33 (+2\%) & 0.35 (+3\%) & 0.36 (+4\%) & CA + timeDist & 0.59 (+18\%) & 0.7 (+8\%) & 0.76 (+5\%) & 0.78 (+5\%) \\
    LR + accEDecayFreq & 0.28 (+35\%) & 0.36 (+12\%) & 0.38 (+12\%) & 0.39 (+12\%) & CA + ALL & 0.56 (+11\%) & 0.68 (+4\%) & 0.73 (+1\%) & 0.75 (+1\%) \\
    LR + avgDecayFreq & 0.28 (+33\%) & 0.36 (+11\%) & 0.37 (+10\%) & 0.38 (+11\%) & LR + timeDist & 0.59 (+18\%) & 0.7 (+8\%) & 0.76 (+5\%) & 0.78 (+5\%) \\
    LR + ALL & 0.23 (+10\%) & 0.31 (-2\%) & 0.34 (+0\%) & 0.35 (+0\%) & LR + ALL & 0.52 (+4\%) & 0.66 (+2\%) & 0.72 (+0\%) & 0.75 (+0\%) \\
    rwrw\_all\_2006-05-07\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-05-07\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.28  & 0.36  & 0.39  & 0.4   & rwrw  & 0.6   & 0.64  & 0.72  & 0.77 \\
    AR + ALL & 0.24 (-15\%) & 0.36 (-2\%) & 0.38 (-4\%) & 0.39 (-4\%) & AR + ALL & 0.47 (-22\%) & 0.6 (-6\%) & 0.68 (-6\%) & 0.74 (-4\%) \\
    CA + accHDecayFreq & 0.32 (+14\%) & 0.38 (+4\%) & 0.4 (+3\%) & 0.42 (+4\%) & CA + timeDist & 0.59 (-2\%) & 0.66 (+3\%) & 0.71 (-1\%) & 0.78 (+1\%) \\
    CA + ALL & 0.29 (+5\%) & 0.37 (+3\%) & 0.39 (-0\%) & 0.41 (+1\%) & CA + ALL & 0.51 (-15\%) & 0.61 (-4\%) & 0.66 (-9\%) & 0.74 (-3\%) \\
    LR + accHDecayFreq & 0.32 (+14\%) & 0.38 (+4\%) & 0.4 (+3\%) & 0.42 (+4\%) & LR + timeDist & 0.59 (-2\%) & 0.66 (+3\%) & 0.71 (-1\%) & 0.78 (+1\%) \\
    LR + ALL & 0.25 (-10\%) & 0.34 (-7\%) & 0.35 (-11\%) & 0.37 (-9\%) & LR + ALL & 0.55 (-9\%) & 0.63 (-1\%) & 0.68 (-5\%) & 0.75 (-3\%) \\
    rwrw\_all\_2006-05-14\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-05-14\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.24  & 0.33  & 0.35  & 0.36  & rwrw  & 0.52  & 0.62  & 0.69  & 0.73 \\
    AR + ALL & 0.27 (+14\%) & 0.37 (+15\%) & 0.39 (+10\%) & 0.4 (+11\%) & AR + ALL & 0.59 (+12\%) & 0.67 (+8\%) & 0.71 (+3\%) & 0.76 (+4\%) \\
    CA + minStrength & 0.29 (+21\%) & 0.39 (+18\%) & 0.4 (+14\%) & 0.41 (+14\%) & CA + accHDecayCE & 0.63 (+21\%) & 0.71 (+15\%)** & 0.74 (+8\%) & 0.77 (+5\%) \\
    CA + ALL & 0.26 (+10\%) & 0.34 (+4\%) & 0.37 (+5\%) & 0.38 (+5\%) & CA + ALL & 0.61 (+16\%) & 0.64 (+3\%) & 0.7 (+1\%) & 0.75 (+2\%) \\
    LR + minStrength & 0.29 (+21\%) & 0.39 (+18\%) & 0.4 (+14\%) & 0.41 (+14\%) & LR + timeDist & 0.58 (+10\%) & 0.68 (+9\%) & 0.72 (+5\%) & 0.77 (+5\%) \\
    LR + ALL & 0.25 (+4\%) & 0.34 (+6\%) & 0.36 (+3\%) & 0.37 (+3\%) & LR + ALL & 0.53 (+2\%) & 0.63 (+2\%) & 0.69 (+0\%) & 0.73 (-0\%) \\
    rwrw\_all\_2006-05-21\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-05-21\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.25  & 0.35  & 0.38  & 0.39  & rwrw  & 0.51  & 0.61  & 0.69  & 0.74 \\
    AR + ALL & 0.28 (+15\%) & 0.4 (+14\%) & 0.42 (+10\%) & 0.42 (+9\%) & AR + ALL & 0.59 (+16\%) & 0.69 (+12\%) & 0.74 (+9\%) & 0.78 (+6\%) \\
    CA + timeDist & 0.29 (+16\%) & 0.4 (+15\%) & 0.42 (+11\%) & 0.42 (+9\%) & CA + timeDist & 0.62 (+22\%) & 0.7 (+14\%)* & 0.75 (+9\%)* & 0.79 (+7\%)* \\
    CA + ALL & 0.25 (+0\%) & 0.35 (-0\%) & 0.38 (0\%) & 0.38 (-1\%) & CA + ALL & 0.55 (+7\%) & 0.63 (+3\%) & 0.69 (+0\%) & 0.74 (-0\%) \\
    LR + timeDist & 0.29 (+16\%) & 0.4 (+15\%) & 0.42 (+11\%) & 0.42 (+9\%) & LR + timeDist & 0.62 (+22\%) & 0.7 (+14\%)* & 0.75 (+9\%)* & 0.79 (+7\%)* \\
    LR + ALL & 0.21 (-17\%) & 0.33 (-5\%) & 0.35 (-7\%) & 0.36 (-7\%) & LR + ALL & 0.48 (-5\%) & 0.63 (+3\%) & 0.68 (-1\%) & 0.73 (-1\%) \\
    rwrw\_all\_2006-05-31\_aol & ERR@1 & ERR@3 & ERR@5 & ERR@10 & rwrw\_all\_2006-05-31\_aol & NDCG@1 & NDCG@3 & NDCG@5 & NDCG@10 \\
    rwrw  & 0.17  & 0.28  & 0.31  & 0.32  & rwrw  & 0.51  & 0.63  & 0.71  & 0.76 \\
    AR + avgDecayCE & 0.25 (+50\%)** & 0.33 (+17\%)* & 0.35 (+14\%) & 0.37 (+14\%)* & AR + ALL & 0.56 (+10\%) & 0.64 (+1\%) & 0.71 (+0\%) & 0.76 (+0\%) \\
    AR + ALL & 0.24 (+44\%)* & 0.32 (+14\%) & 0.35 (+13\%) & 0.36 (+12\%) & CA + maxDuration & 0.6 (+18\%) & 0.67 (+6\%) & 0.74 (+4\%) & 0.79 (+4\%) \\
    CA + ALL & 0.25 (+48\%)* & 0.31 (+11\%) & 0.33 (+8\%) & 0.35 (+9\%) & CA + ALL & 0.58 (+14\%) & 0.65 (+2\%) & 0.7 (-1\%) & 0.76 (+1\%) \\
    LR + avgDecayCE & 0.25 (+50\%)** & 0.33 (+17\%)* & 0.35 (+14\%)* & 0.37 (+14\%)* & LR + maxDuration & 0.6 (+18\%) & 0.67 (+6\%) & 0.74 (+4\%) & 0.79 (+4\%) \\
    LR + ALL & 0.17 (+1\%) & 0.28 (-2\%) & 0.3 (-3\%) & 0.31 (-2\%) & LR + ALL & 0.48 (-5\%) & 0.61 (-3\%) & 0.67 (-5\%) & 0.74 (-3\%) \\
    \bottomrule
    \end{tabular}%
  \label{tab:rwrwallfix}%
\end{table}%

